Accelerated Inchworm Method with Tensor-Train Bath Influence Functional

We propose an efficient tensor-train-based algorithm for simulating open quantum systems with the inchworm method, where the reduced dynamics of the open quantum system is expressed as a perturbative series of high-dimensional integrals. Instead of evaluating the integrals with Monte Carlo methods, we approximate the costly bath influence functional (BIF) in the integrand as a tensor train, allowing accurate deterministic numerical quadrature schemes implemented in an iterative manner. Thanks to the low-rank structure of the tensor train, our proposed method has a complexity that scales linearly with the number of dimensions. Our method couples seamlessly with the tensor transfer method, allowing long-time simulations of the dynamics.

==> section_5.tex <==
% \zc{I suggest further simplification of this section because it is not a part of our work. We need to explain the motivation of using TTM, which is the growth of bond dimensions with respect to time, but for the details, I think it is enough to say that $\rho_s(t_k) = \sum_{j=1}^{K_{\max}} \mathcal{T}_k \rho_s(t_{k-j})$, and the transfer tensors $\mathcal{T}_k$ is learned from the evolution of the first $K_{\max}$ time steps for all bases of the initial density matrix.}
% \ki{I think we may delete the whole section and simply introduce TTM in the numerical test section.}
% In the last section, we can observe that the computational cost of our method relies heavily on the bond dimensions of the BIF-TTs, which in turn depend on the rank $r$ of the TPCM.
% When the number of time steps $N$ increase, the rank $r$ of the TPCM also increases.
% Therefore, the computational cost grows fast for longer-time simulations.
% To overcome this difficulty, we can apply the transfer tensor method (TTM) \cite{cerrillo2014nonmarkovian} in our numerical simulation.
% TTM can be regarded as a discretization of Nakajima-Zwanzig equation \cite{nakajima1958quantum,zwanzig1960ensemble}. 
% TTM assumes a finite time correlation for the non-Markovian system.
% By computing the dynamical maps and transfer tensors, TTM allows long time simulation based on short time transfer tensors.

% Assume $t_k=k\Delta t$, the non-Markovian open quantum trajectories generate dynamical maps that propagate the reduced density matrix
% \begin{equation}
%     \rho_s(t_k) = \mathcal{E}_k \rho_s(0)
% \end{equation}
% with $\mathcal{E}_k$ being the dynamical maps for $k$ steps.
% It is clear that $\mathcal{E}_0$ is the identical map.
% The dynamical maps are then decomposed to
% \begin{equation}
% \label{eq_transfer_tensor_to_dynamical_maps}
%     \mathcal{E}_k = \sum_{j=1}^{k} \mathcal{T}_{j} \mathcal{E}_{k-j} 
% \end{equation}
% where $\mathcal{T}_j$ are called transfer tensors.
% Since the sequence of transfer tensors decays, \emph{i.e.},
% \begin{equation}
%     \lim_{j\rightarrow \infty} \Vert \mathcal{T}_{j} \Vert = 0,
% \end{equation}
% we may set a memory length $K_{\max}$ such that when $j>K_{\max}$, the transfer tensors are ignored.
% Therefore, for $k>K_{\max}$, the dynamical maps are given approximately by 
% \begin{equation}
% \label{eq_TTM_propagate}
%     \mathcal{E}_k = \sum_{j=1}^{K_{\max}} \mathcal{T}_j \mathcal{E}_{k-j}.
% \end{equation}
% In conclusion, there are two steps in TTM.
% In the learning procedure, we need to construct dynamical maps $\mathcal{E}_j$ and the transfer tensors $\mathcal{T}_j$ for $j=1,\cdots, K_{\max}$. 
% The dynamical maps can be obtained from experiments or other numerical methods.
% In this paper, when we apply TTM, the dynamical maps are constructed by the tensor train based inchworm algorithm introduced in the following sections with different initial reduced density operators.
% With the dynamical maps, the transfer tensors can be computed by the equivalent form of \cref{eq_transfer_tensor_to_dynamical_maps}
% \begin{equation}
%     \mathcal{T}_k = \mathcal{E}_k - \sum_{j=1}^{k-1} \mathcal{T}_j \mathcal{E}_{k-j}.
% \end{equation}
% In the propagating procedure, we apply \cref{eq_TTM_propagate} for the long time simulation.

% The following part focuses on the construction of dynamical maps within the memory length.
% By \cref{eq_full_propagator}, we may compute the full propagator for the observable on the system $O_s$.
% If we choose an artificial observable $O=E_{ij}\otimes \id_b$ with $E_{ij}$ being the matrix unit at $(i,j)$.
% This observable is called ``artificial'' because it does not have a physical meaning like other observables.
% The idea is similar to the splitting of observables into basic operators in \cite{cai2023bold}.
% The reason to use this artificial observables is that they help with the construction of dynamical maps.
% When we choose the observable as $E_{ij}\otimes \id_b$, the resulting $G_{-k,k}$ gives us the elements of the dynamical maps in $\mathcal{E}_k$.
% By choosing all possible $(i,j)$ pairs, we can construct the full dynamical maps with the method proposed in the paper.
% \yx{Maybe we can write this in equations? 
% \begin{equation*}
%     \expval{O(t)}=\tr\left(O_s\otimes I_{\mathrm{b}}\rho(t)\right)=\tr_{s}\left(O_s\rho_{s}(t)\right)=\tr_{s}\left(O_s\mathcal{E}(t)\rho_{s}(0)\right)
% \end{equation*}
% If we denote the $O_{s}$, $\rho_{s}$ and $\mathcal{E}$ in vectorized Liouville space as $\hat{O}_{s}$, $\hat{\rho}_{s}$ and $\hat{\mathcal{E}}$. Here the super-operator $\mathcal{E}$ has become a $4\times 4$ matrix $\hat{\mathcal{E}}$. Therefore,
% \begin{equation*}
% \expval{O(t)}=\hat{O}_{s}^\dagger \hat{\mathcal{E}}(t)\hat{\rho}_{s}(0)
% \end{equation*}
% By choosing the vectorized $\hat{O}_s$ and $\rho_{s}$ to be unit vectors, then the output $\expval{O(t)}_{i,j}=e_i^\dagger\hat{\mathcal{E}}e_j$ is exactly the $(i,j)$ component of $\hat{\mathcal{E}}(t)$.
% }
% After constructing the dynamical maps $\mathcal{E}_k$ within the memory length, we can then following the procedure of TTM to construct dynamical maps and perform long time simulation of the system. 
% Clearly, the rank $r$ of the TPCM is relatively small when a small number of time steps $N$ is required, further yields small bond dimensions in the BIF-TTs.
% The computational cost is, therefore, under control.


